Progressive Multi-granular Alignments for Grounded Reasoning in Large Vision-Language Models

Existing Large Vision-Language Models (LVLMs) excel at matching concepts across multi-modal inputs but struggle with compositional concepts and high-level relationships between entities. This paper introduces Progressive multi-granular Vision-Language alignments (PromViL), a novel framework to enhance LVLMs' ability in performing grounded compositional visual reasoning tasks. Our approach constructs a hierarchical structure of multi-modal alignments, ranging from simple to complex concepts. By progressively aligning textual descriptions with corresponding visual regions, our model learns to leverage contextual information from lower levels to inform higher-level reasoning. To facilitate this learning process, we introduce a data generation process that creates a novel dataset derived from Visual Genome, providing a wide range of nested compositional vision-language pairs. Experimental results demonstrate that our PromViL framework significantly outperforms baselines on various visual grounding and compositional question answering tasks. The code is available at: https://github.com/lqh52/PromViL.

==> reproducibility_checklist.tex <==
This paper:
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI
methods introduced: yes
\item Clearly delineates statements that are opinions, hypothesis, and speculation
from objective facts and results: yes
\item Provides well marked pedagogical references for less-familiare readers
to gain background necessary to replicate the paper: yes
\end{itemize}
Does this paper make theoretical contributions? no

Does this paper rely on one or more datasets? yes
\begin{itemize}
\item A motivation is given for why the experiments are conducted on the
selected datasets: yes
\item All novel datasets introduced in this paper are included in a data
appendix: no
\item All novel datasets introduced in this paper will be made publicly
available upon publication of the paper with a license that allows
free usage for research purposes: yes
\item All datasets drawn from the existing literature (potentially including
authors\textquoteright{} own previously published work) are accompanied
by appropriate citations: yes
\item All datasets drawn from the existing literature (potentially including
authors\textquoteright{} own previously published work) are publicly
available: yes
\item All datasets that are not publicly available are described in detail,
with explanation why publicly available alternatives are not scientifically
satisficing: NA
\end{itemize}
Does this paper include computational experiments? yes
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix:
yes
\item All source code required for conducting and analyzing the experiments
is included in a code appendix: yes
\item All source code required for conducting and analyzing the experiments
will be made publicly available upon publication of the paper with
a license that allows free usage for research purposes: yes
\item All source code implementing new methods have comments detailing the
implementation, with references to the paper where each step comes
from: yes
\item If an algorithm depends on randomness, then the method used for setting
seeds is described in a way sufficient to allow replication of results:
yes
\item This paper specifies the computing infrastructure used for running
experiments (hardware and software), including GPU/CPU models; amount
of memory; operating system; names and versions of relevant software
libraries and frameworks: yes
\item This paper formally describes evaluation metrics used and explains
the motivation for choosing these metrics: yes
\item This paper states the number of algorithm runs used to compute each
reported result: yes
\item Analysis of experiments goes beyond single-dimensional summaries of
performance (e.g., average; median) to include measures of variation,
confidence, or other distributional information: no
\item The significance of any improvement or decrease in performance is
judged using appropriate statistical tests: no
\item This paper lists all final (hyper-)parameters used for each model/algorithm
in the paper\textquoteright s experiments: yes
\item This paper states the number and range of values tried per (hyper-)
parameter during development of the paper, along with the criterion
used for selecting the final parameter setting: NA
\end{itemize}


